When Being Unseen from mBERT is just the Beginning: Handling New Languages With Multilingual Language Models

Transfer learning based on pretraining language models on a large amount of raw data has become a new norm to reach state-of-the-art performance in NLP. Still, it remains unclear how this approach should be applied for unseen languages that are not covered by any available large-scale multilingual language model and for which only a small amount of raw data is generally available. In this work, by comparing multilingual and monolingual models, we show that such models behave in multiple ways on unseen languages. Some languages greatly benefit from transfer learning and behave similarly to closely related high resource languages whereas others apparently do not. Focusing on the latter, we show that this failure to transfer is largely related to the impact of the script used to write such languages. Transliterating those languages improves very significantly the ability of large-scale multilingual language models on downstream tasks.

==> Makefile <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = naccl-2021
#emnlp2020_with_iffalses_and_commented_parts
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles =  benoit_translit.tex



















#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).pdf 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	rm -f $(latexfile).toc
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex &


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp: 
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours/$(latexfile)_draft.pdf

ebib:
	open $(latexfile).bib

cloud: pdf
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/A\ Lire\ -\ iCloud/




==> Makefile_ <==
# set latexfile to the name of the main file without the .tex
#latexfile = eacltest
latexfile = arxiv-202010
#emnlp2020_with_iffalses_and_commented_parts
# put the names of figure files here.  include the .eps
figures = 

#includedfiles = Intro.tex State-of-the-art.tex Experiments.tex Discussion.tex
includedfiles =  benoit_translit.tex



















#Algos.tex Discussion.tex Results.tex \
#	eacltest.tex experiences.tex intro.tex lexical-inpact.tex \
#	presentation-treebank.tex protocol.tex state-of-the-art-comparaison.tex\
#	corpus-setup-experiment.tex TODO.tex Tagset.tex crossparsing.tex \
#	new_intro.tex new_presTB.tex new_protocol.tex examples-marie.tex

TEX = pdflatex

# *.fig files may be in ./Figs
vpath %.fig Figs


all: pdf
$(latexfile).dvi : $(figures) $(includedfiles) $(latexfile).tex


%.eps : %.fig
	fig2dev -L eps $< > $@

$(latexfile).pdf : $(latexfile).tex $(includedfiles) $(figures)
	$(TEX)  $(latexfile).tex
#	$(TEX)  appendix.tex

pdf :	$(latexfile).pdf 

bib : $(latexfile).tex
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
	bibtex $(latexfile)
	$(TEX) $(latexfile)
	$(TEX) $(latexfile)
#	$(TEX) $(latexfile)
	
	 
force:
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

appendix.pdf: 
	$(TEX)  appendix.tex
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix
	bibtex appendix
	$(TEX) appendix
	$(TEX) appendix

	

$(latexfile).ps : $(latexfile).dvi
	dvips  -Ppdf $(latexfile) -o $(latexfile).ps

ps : $(latexfile).ps 

$(latexfile).tar.gz : $(figures) $(latexfile).tex
	tar -czvf $(latexfile).tar.gz $(figures) $(latexfile).tex Figs/*.fig

tarball: $(latexfile).tar.gz


clean: 
	rm -f $(latexfile).bbl
	rm -f $(latexfile).log
	rm -f $(latexfile).dvi
	rm -f $(latexfile).blg
	rm -f $(latexfile).aux
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf
	rm -f $(latexfile).out
	rm -f $(latexfile).toc
	
clean2:
	rm -f appendix.bbl
	rm -f appendix.log
	rm -f appendix.dvi
	rm -f appendix.blg
	rm -f appendix.aux
	rm -f appendix.ps
	rm -f appendix.pdf
		
check:
	cat $(latexfile).log | grep --text undef

dist-clean: clean
	rm -f $(latexfile).ps
	rm -f $(latexfile).pdf

viewX: pdf 
	open $(latexfile).pdf
	
viewA: pdf
	open -a Preview.app $(latexfile).pdf

view: pdf
	open -a Skim.app $(latexfile).pdf
#	open -a Skim.app appendix.pdf 

gv: ps
	gv $(latexfile).pdf


edit: 
	xemacs $(latexfile).tex &


up:
	git pull

co:	commit
	
commit:
	git commit -m "update" 	./
	git push

commitsvn:
	svn commit -m "update" ./

upsvn:
	svn up

cp: 
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/PapiersEnCours/$(latexfile)_draft.pdf

ebib:
	open $(latexfile).bib

cloud: pdf
	cp $(latexfile).pdf /Users/djame2/Library/Mobile\ Documents/3L68KQB4HG~com~readdle~CommonDocuments/Documents/A\ Lire\ -\ iCloud/




==> datanotes.tex <==
\begin{table*}[h!]
    \centering\footnotesize
    \begin{tabular}{lccccccc}
    Language [ISO 639-1/2]& XLM-R & mBERT & UD & WikiANN & Oscar & G-Translate & Tatoeba\\
    \midrule
Abaza [abq] &Out & Out & In & Out & Out \\
Akkadian [akk] & Out & Out & In &  Out & Out\\
Amharic [am] & In & Out & In & In &In & In & In-212s\\
Ancient Greek & Out & Out  & In & Out &  Out \\
Assamese [as] & In & Out & Out & In & In \\
Assyrian [aii] & Out & Out & In & Out &Out \\
Bambara & Out & Out  &  In-ish & Out & Out & Out \\
Bhojpuri [bho] & Out & Out  & In & Out & Out\\
Buryat & Out & Out  & In & Out & Out\\
Cebuano [ceb] & Out & In & Out & In & In & In & In\\
Coptic & Out & Out & In & Out& Out \\
Dhivehi [dv] & Out & Out & Out & In & In \\
Erzya & Out & Out & In & Out & Out-78w\\
Faroese [fo] & Out & Out & In & In & Out \\
Gothic & Out & Out & In &Out & Out\\
Karelian [krl]& Out & Out & In & Out & Out \\
Komi Permyak & Out & Out  & In  & Out & Komi?\\
Komi Zyrian [kpv] & Out & Out  & In & Out & Komi?  \\
Central Khmer [km] & In & Out & Out & In & In & In \\
Kurmanji (Northen Kurdish) [ku] & In & Out  & In & In & Kurdish? & In & In\\
Livvi & Out & Out  & In & Out & Out \\
Magahi [mag] & Out & Out  & MISSING & Out & Out\\
Maltese [mt] & Out & Out & In & In & In & In & In-200s\\
Mbya Guarani [gun] & Out & Out  & In & Out  & Out\\
Moksha & Out & Out  & In & Out & Out \\
Naija & Out & Out  & In & Out & Out \\
North Sami & Out & Out  & In & Out & Out & In-145s\\
Old Church Slavonic & Out & Out  & In & Out & Out \\
Old French  & Out & Out  & In & Out & Out \\
Old Irish &  Out & Out & In & Out & Out\\
Old Russian  & Out & Out & In & Out & Out \\
Sanskrit [sa] & In & Out & In & Out & In\\
Scottish Gaellic [gd] & In & Out  & In & In & In & In\\
Sindhi [sd] & In & Out & missing & In & In & In \\
Skolt Sami & Out & Out  & In & Out & Out \\
Swiss German [gsw] & Out & Out  & In & Out & Out \\
Tagalog [tl] & In & In  & In & In & In & In \\
Upper Sorbian [hsb] & Out & Out  & In & In & In \\
Uyghur [ug] & In & Out  & In & In & In & In\\
Warlpiri & Out & Out  & In & Out & Out\\
Wolof [wo] & Out & Out  & In & Out & Out\\
Yoruba [yo] & Out & In  & In & Out & In & In \\
\bottomrule
    \end{tabular}
    \caption{Languages not included in at least one of the pretraining corpora of mBERT and XLM-R ()}
    \label{tab:ressource}
\end{table*}


==> figs/langs-2.tex <==


\begin{table}[ht!]
\footnotesize\centering
\scalebox{0.92}{ % was .7775
\begin{tabular}{lrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
    
    Language & Script & Family & \#sents \\%& \\
    \midrule
    Bambara & Latin & Niger-Congo& 1k\\
    Wolof  & Latin & Niger-Congo & 10k\\
    %Kurmanji & Latin & Kurdish & 105k\\
    Swiss & Latin & Germanic & 250k\\
    Naija & Latin & English Pidgin & 237k \\
    Faroese & Latin & Scandinavian&297k \\
    Maltese & Latin & Siculo-Arabic & 50k \\
    Narabizi & Latin & Arabic* & 87k\\
    Sorani & Arabic & Kurdish & 380k\\
    Uyghur & Arabic & Turkic &  105k\\
    Sindhi & Arabic & Indo-Aryan & 375k\\
    Mingrelians (xmf) & Georgian & Kartvelian & 29k\\
    Buryat & Cyrillic & Mongolic & 7k\\
    Meadow Mari (mhr) & Cyrillic & Uralic & 58k\\
    Erzya (myv) & Cyrillic & Uralic &  20k\\
    Livvi (olo) & Latin & Uralic &  9.4k\\
    %Min Dong? (cdo)& Latin & Sinitic \\
    
    
    
    

    
\bottomrule
\end{tabular}
}
%}
\caption{\textit{Unseen} Languages used for downstream experiments. \#sents indicates the number of raw sentences (based on the OSCAR corpus \citep{OrtizSuarezSagotRomary2019} except for Faroese and Narabizi) used for \mlmtuning \\ 
\small{*code-mixed with French }}
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
\label{tab:langs}
\end{table}


==> figs/mlm_on_unseen.tex <==

\begin{table*}[ht]
\small\centering
\resizebox{\linewidth}{!}{
\begin{tabu}{ l  c  c c c@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c  c c c@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c  c c c}%@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c  c }
	\toprule
	& \multicolumn{4}{c @{\hspace{0.5cm}}}{\textsc{UPOS}} & \multicolumn{4}{c @{\hspace{0.7cm}}}{\textsc{LAS}} & \multicolumn{4}{c @{\hspace{0.7cm}}}{\textsc{NER}} & %\multicolumn{3}{c @{\hspace{0.35cm}}}{\textsc{ParTUT}} \\
	\cmidrule(l{2pt}r{0.4cm}){2-5}\cmidrule(l{-0.2cm}r{0.4cm}){6-9}\cmidrule(l{-0.2cm}r{0.4cm}){10-13}%\cmidrule(l{-0.2cm}r{2pt}){8-9}
	\multirow{-2}{*}[1pt]{Model} & 
	\textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm & Baseline 
	%\multirow{-2}{*}[1pt]{}
	& \textsc{\mbert}   &\textsc{\mbertmlm} & \monomlm & Baseline 
	%\multirow{-2}{*}[1pt]{} 
	& \textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm & Baseline 
	\\
	\midrule
	\textit{Easy}\\
	%benjamin t'es lo ? ???
	Faroese \textit{few-shots} & 96.31 & 96.52     & 91.12& 95.36 & 84.02 & 86.42 & 67.66 & 83.11 & 52.11   & \bf 58.34 & 39.33 & 50.11  \\ 
	%Faroese (src:scand) & 
	% POS 79.39 & 83.41 & 66.44 & &%77.46(udif) &
	% LAS  67.50 & 69.81 & 35.82 &- &%59.26(udif) &
	%35.82 & x & x & x &
	% NER 
	Naija & 
	% POS
	89.27 & 89.56 & 87.1 & 89.21 &
	% LAS 
	71.55 & 69.19 & 63.02 & 68.32 &
	% NER 
	- & - & - & - & 
	Swiss German \textit{few-shots} & 76.66 & 78.68  & 65.42 & 75.22 &  35.68 & 42.32 & 26.47  & 32.18\\
	%Swiss German (src:De)    & 
	% POS 
	% 62.67 & 87.92 &64.65 & - & 
	% LAS 
	% 41.22 & 69.58 &  29.97 & - & 
	% NER 
	% - &  - & - & - &
	 
	 


	\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
	\textit{Intermediate}\\
	
	Maltese & 
	% POS
	% x.  & x     & x     &    &
	92.04 & \bf 96.38 & 92.05 &  95.99 & 
	% Parsing
	74.41 & \bf 82.15 & 66.55 & 79.71 & 
	% NER 
	61.23 & \bf 66.75 & 62.56 & 63.10 &
	
% XLM-R cf. table 5
	
	
	Narabizi &
	  % POS
	  81.60  & \bf 84.22  &  71.35  &  84.20 &
	  % LAS
	  56.52  & \bf 57.83  &  41.78  &  52.84 &
	  % NER 
	  -  & -  &  -  &  -  &
	Sindhi & 
	% POS
	-  & -  &  -  &  -  &
	% LAS
	-  & -  &  -  &  -  &
	% NER
	42.27  & \bf 47.93  &  45.18  &  44.10  &
	
	Bambara \textit{few-shots}&  90.23 & 92.57 & 78.09 & 92.32 &  71.84 & 75.37  & 46.43   & 76.21 & -  & - & - \\
    Wolof &  92.85 & \bf 95.22 &88.41 &94.09 & 73.26&\bf 77.91& 62.80& 77.05 & - & - & - & -\\

	\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
	\textit{Hard}\\
	%Amharic(?) & \\
	Sorani & 
	% POS
	 -  & -  &  -  &  -  &
	% LAS 
	 -  & -  &  -  &  -  &
	% NER 
	70.45  & 75.56  &  \bf 80.58  &  81.31  &
	%Kurmanji  & 
	% POS
	%   54.71 & x  &  x  &  x  &
	% LAS 
	% 11.83 & x &  x &  x  &
	% NER 
	%-  & -  &  -  &  -  &
	
	Uyghur & 
	% POS
	 76.98  & 77.33  &    87.39  &  \bf 89.87  &
	 % LAS
	 45.47  & 48.91  &   57.29  &   \bf 67.09  &
	 % NER
	 24.32  & 34.66  &  \bf 41.42  &  50.12  &
	%\camembert (fine-tuned)                           & \textbf{98.18}    & \textbf{92.57}    & \underline{99.29}          & \textbf{94.20}    & 96.99             & 81.37             & \textbf{97.65}    & \textbf{93.43}             \\ % 10125734 : POS best seed PARSING gsd 10126431 PARSING other : 10126429
	%UDPipe Future \mbox{+ \camembert} (embeddings)    & 97.96             & 90.57             & 99.25          & \underline{93.89}             & \underline{97.09}             & \textbf{81.81}             & 97.50             & 92.32             \\
	

	 
	\bottomrule
	
\end{tabu}
}
\caption{\textbf{POS}, \textbf{Dependency Parsing} and \textbf{NER} scores comparing \mbert and \mbertmlm  to \monomlm, a language model trained from scratch on the available raw data in the target language, and a strong non-contextual baseline (for POS and Parsing the baseline is udpipe future, % (except for Narabizi for which it is StanfordNLP)
for NER it is a LSTM-CRF model)
% INFO MLM data: 
% Narabizi : 50k from Seddah 
% Maltese: +MLM oscar (MLM only 5M from leipzig, need to fix this) 
%
}%
\label{tab:mlm_on_unseen}
\end{table*}

==> figs/parsing_cross_lingual.tex <==


\begin{table*}[b]
\footnotesize\centering
\scalebox{0.8}{ % was .7775
\begin{tabular}{lrrrrrrrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     Target~/~Source & \multicolumn{1}{c}{\textsc{En}} &  \multicolumn{1}{c}{\textsc{De}} & \multicolumn{1}{c}{\textsc{Go}} & \multicolumn{1}{c}{\textsc{FR}} & \multicolumn{1}{c}{\textsc{Fr}} & \multicolumn{1}{c}{\textsc{O-Fr}} & \multicolumn{1}{c}{\textsc{It}} & \multicolumn{1}{c}{\textsc{Ru}} & \multicolumn{1}{c}{\textsc{O-Ru}} & \multicolumn{1}{c}{\textsc{Tu}} & \multicolumn{1}{c}{\textsc{Uy}} & \multicolumn{1}{c}{\textsc{Ar}} & \multicolumn{1}{c}{\textsc{Narz}} & \multicolumn{1}{c}{\textsc{Mt}} \\
     \midrule
     \\
\textsc{English} & \cellcolor{lightgreen}88.62 & 65.77 & 17.00 & 60.67 & 76.86 & 44.13 & 79.22 && 27.20 && 5.66 & 25.27 & 28.72 & 10.86 \\ 
\textsc{Naija} & 28.58 & 25.48 & 8.19 & 22.29 & 31.40 & 14.84 & 28.06 && 10.42 && 7.92 & 10.21 & 18.47 & 7.25 \\ 
\textsc{German} & 63.54 & \cellcolor{lightgreen}74.50 & 21.39 & 61.68 & 67.12 & 43.94 & 67.87 && 31.18 && 9.24 & 24.41 & 30.83 & 32.58 \\ 
\textsc{Gothic} & 7.47 & 10.37 & \cellcolor{lightgreen}63.40 & 8.01 & 9.34 & 10.87 & 10.28 && 7.32 && 3.30  &10.08 & 11.21 & 6.75 \\ 
\textsc{French} & 70.09 & 59.61 & 19.07 & \cellcolor{lightgreen}86.40 & 73.73 & 43.08 & 72.71 && 26.00 && 4.99 & 25.49 & 39.90 & 34.20 \\ 
\textsc{French Partut} & 82.51 & 69.55 & 23.22 & 74.91 & \cellcolor{lightgreen}90.78 & 50.15 & 86.33 && 31.69 && 5.40 & 26.07 & 42.14 & 38.36 \\ 
\textsc{Old French} & 34.09 & 35.16 & 20.13 & 37.24 & 40.46 & \cellcolor{lightgreen}64.09 & 36.16 && 24.40 && 6.44 & 16.39 & 25.60 & 15.79 \\ 
\textsc{Italian} & 82.36 & 67.06 & 23.04 & 75.23 & 84.25 & 47.09 & \cellcolor{lightgreen}90.02 && 31.30 && 5.05 & 27.32 & 41.21 & 44.90 \\ 
\textsc{Russian} & 62.33 & 54.03 & 15.52 & 58.61 & 56.81 & 27.80 & 61.92 && 28.97 && 5.81 & 35.70 & 21.98 & 27.15 \\ 
\textsc{Old Russian} & 22.27 & 24.47 & 18.73 & 25.18 & 24.34 & 22.46 & 28.63 && \cellcolor{lightgreen}43.97 && 4.85 & 20.37 & 17.82 & 18.24 \\ 
\textsc{Turkish} & 30.38 & 26.80 & 7.63 & 25.11 & 26.55 & 14.61 & 27.87 && 13.82 && 18.30 & 11.70 & 11.58 & 10.03 \\ 
\textsc{Uyghur} & 6.45 & 4.91 & 1.32 & 3.60 & 4.23 & 1.41 & 4.75 && 0.35 && \cellcolor{lightgreen}43.78 & 4.48 & 4.14 & 3.58 \\ 
\textsc{Arabic} & 25.28 & 17.84 & 11.73 & 27.05 & 25.89 & 8.79 & 27.65 && 12.29 && 2.24 & \cellcolor{lightgreen}71.82 & 14.71 & 16.44 \\ 
\textsc{Arabizi} & 16.01 & 15.94 & 10.64 & 17.21 & 18.87 & 12.35 & 18.17 && 5.77 && 1.71 & 9.11 & \cellcolor{lightgreen}51.35 & 17.27 \\ 
\textsc{Maltese} & 7.15 & 8.89 & 3.03 & 6.40 & 8.52 & 5.53 & 11.01 && 1.38 && 2.15 & 5.32 & 11.43 & \cellcolor{lightgreen}70.49 \\ 
\textsc{Bambara} & 9.19 & 6.94 & 2.07 & 6.39 & 7.90 & 2.26 & 6.01 && 1.68 && 6.97 & 5.56 & 5.28 & 6.54 \\
    \bottomrule
\end{tabular}
}
\caption{Cross-Lingual performance of \mbert Parsing (LAS score) (\colorbox{lightgreen}{In-Distribution} performances) 1,500 training sentences at most 
}

\label{tab:parsing_cross_lingual_2}
\end{table*}

==> figs/pos_cross_lingual.tex <==


\begin{table*}[b]
\footnotesize\centering
\scalebox{0.8}{ % was .7775
\begin{tabular}{lrrrrrrrrrrrrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     Target~/~Source & \multicolumn{1}{c}{\textsc{En}} &  \multicolumn{1}{c}{\textsc{De}} & \multicolumn{1}{c}{\textsc{Go}} & \multicolumn{1}{c}{\textsc{FR}} & \multicolumn{1}{c}{\textsc{Fr}} & \multicolumn{1}{c}{\textsc{O-Fr}} & \multicolumn{1}{c}{\textsc{It}} & \multicolumn{1}{c}{\textsc{Ru}} & \multicolumn{1}{c}{\textsc{O-Ru}} & \multicolumn{1}{c}{\textsc{Tu}} & \multicolumn{1}{c}{\textsc{Uy}} & \multicolumn{1}{c}{\textsc{Ar}} & \multicolumn{1}{c}{\textsc{Narz}} & \multicolumn{1}{c}{\textsc{Mt}} \\
     \midrule
     \\
\textsc{English} & \cellcolor{lightgreen}95.99 & 87.43 & 48.87 & 86.03 & 90.68 & 68.79 & 89.20 & 82.97 & 63.09 & 63.78 & 34.55 & 65.24 & 72.64 & 18.85 \\ 
\textsc{Naija} & 69.72 & 63.86 & 30.55 & 44.52 & 70.19 & 41.16 & 67.30 & 25.92 & 37.60 & 54.71 & 40.33 & 43.54 & 57.68 & 28.29 \\ 
\textsc{German} & 89.35 & \cellcolor{lightgreen}94.57 & 47.16 & 86.41 & 88.65 & 65.34 & 87.34 & 81.81 & 58.94 & 68.81 & 39.08 & 61.78 & 71.81 & 61.50 \\ 
\textsc{Gothic} & 28.38 & 26.17 & \cellcolor{lightgreen}91.60 & 20.06 & 29.14 & 34.16 & 31.43 & 9.47 & 13.21 & 24.80 & 20.48 & 11.21 & 25.47 & 28.89 \\ 
\textsc{French} & 90.46 & 85.97 & 52.10 & \cellcolor{lightgreen}96.82 & 94.15 & 73.33 & 93.43 & 82.00 & 59.41 & 64.27 & 34.41 & 61.68 & 81.20 & 63.79 \\ 
\textsc{French Partut} & 93.32 & 87.57 & 53.02 & 94.03 & \cellcolor{lightgreen}97.52 & 77.01 & 95.12 & 83.58 & 62.97 & 62.26 & 33.19 & 64.60 & 80.10 & 66.73 \\ 
\textsc{Old French} & 62.68 & 57.39 & 47.30 & 66.96 & 63.59 & \cellcolor{lightgreen}87.78 & 62.78 & 50.24 & 52.03 & 44.20 & 21.53 & 35.11 & 61.03 & 35.85 \\ 
\textsc{Italian} & 92.82 & 88.23 & 57.23 & 94.30 & 94.81 & 77.45 & \cellcolor{lightgreen}97.79 & 85.08 & 66.41 & 64.31 & 32.73 & 66.79 & 80.78 & 71.99 \\ 
\textsc{Russian} & 86.56 & 82.74 & 49.70 & 84.12 & 83.92 & 60.48 & 84.36 & \cellcolor{lightgreen}97.49 & 63.72 & 71.41 & 41.49 & 72.11 & 67.95 & 63.79 \\ 
\textsc{Old Russian} & 49.09 & 45.90 & 46.57 & 50.34 & 50.98 & 52.47 & 54.19 & 46.42 & \cellcolor{lightgreen}72.46 & 41.33 & 23.78 & 37.99 & 47.09 & 40.40 \\ 
\textsc{Turkish} & 73.28 & 66.84 & 41.13 & 70.41 & 73.16 & 48.03 & 71.56 & 73.17 & 48.94 & \cellcolor{lightgreen}93.07 & 53.71 & 57.01 & 53.74 & 57.36 \\ 
\textsc{Uyghur} & 21.45 & 30.74 & 21.12 & 21.26 & 23.27 & 14.26 & 23.43 & 27.25 & 2.80 & 37.91 & \cellcolor{lightgreen}73.75 & 22.03 & 28.90 & 32.85 \\ 
\textsc{Arabic} & 61.97 & 62.89 & 48.72 & 62.93 & 64.45 & 49.21 & 63.89 & 73.66 & 66.08 & 53.57 & 36.11 & \cellcolor{lightgreen}95.16 & 61.11 & 53.03 \\ 
\textsc{Arabizi} & 37.65 & 33.48 & 28.23 & 34.64 & 36.60 & 36.21 & 37.11 & 21.77 & 16.70 & 28.33 & 20.03 & 19.23 & \cellcolor{lightgreen}81.60 & 34.60 \\ 
\textsc{Maltese} & 31.33 & 31.82 & 20.83 & 26.61 & 30.54 & 23.53 & 32.73 & 24.64 & 6.63 & 31.34 & 28.47 & 18.75 & 42.28 & \cellcolor{lightgreen}93.34 \\ 
\textsc{Bambara} & 35.47 & 27.93 & 14.03 & 34.21 & 34.47 & 12.11 & 31.64 & 30.14 & 5.24 & 31.64 & 33.13 & 20.57 & 22.99 & 26.48 \\
     
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer & 

    \bottomrule
\end{tabular}
}
\caption{Cross-Lingual performance of \mbert POS (\colorbox{lightgreen}{In-Distribution
} performances)
1,500 training sentences at most 
% 10433845 job 
}
\label{tab:pos_cross_lingual}
\end{table*}



==> figs/single_lang_tables/bambara.tex <==
\begin{table}[htbp]
    \centering\small
    \begin{tabular}{lccc}
    \toprule
        Model & UPOS & LAS \\
    \midrule
        Baseline & \textbf{92.3} & \textbf{76.2}\\        BambaraBERT & 78.1 & 46.4 \\
        \mbert & 90.2 & 71.4\\
        \mbert+MLM & \textbf{92.6} & \textbf{75.4}\\
    \bottomrule
    \end{tabular}
    \caption{Bambara also falls into the Intermediate category. \mlmtuning enables \mbert to match outperform the strong non-contextual baseline in POS tagging}
    \label{tab:bambara}
\end{table}

==> figs/single_lang_tables/maltese.tex <==

\begin{table}[htbp]
    \centering\small
    \begin{tabular}{lccc}
    \toprule
        Model & UPOS & LAS & NER \\
    \midrule
        Baseline & 95.99 & 79.71 & 65.1 \\
        MalteseBERT & 92.1 & 66.5 & 62.5 \\
        \mbert & 92.0 & 74.4 & 61.2\\
        \mbert+MLM & \textbf{96.4} & \textbf{82.2} & \textbf{66.7}\\
    \bottomrule
    \end{tabular}
    \caption{Maltese is an ``Intermediate'' unseen language: a multilingual model requires language-specific MLM and task-tuning to achieve performance  competitive to a monolingual baseline.}
    \label{tab:maltese}
\end{table}

==> figs/single_lang_tables/narabizi.tex <==
\begin{table}[htbp]
    \centering\small
    \begin{tabular}{lccc}
    \toprule
        Model & UPOS & LAS \\
    \midrule
        Baseline & \textbf{84.20} & 52.84\\        NarabiziBERT & 71.3 & 52.8 \\
        \mbert & 81.6 & 56.5\\
        \mbert+MLM & \textbf{84.22} & \textbf{57.8}\\
    \bottomrule
    \end{tabular}
    \caption{Narabizi falls into the Intermediate category. \mlmtuning enables \mbert to match or outperform strong non-contextual baselines}%the results for POS tagging fall into the ``Intermediate'' pattern, but for DEP fall in the ``easy'' unseen languages pattern.}
    \label{tab:narabizi}
\end{table}


==> figs/single_lang_tables/uyghur.tex <==

\begin{table}[t!]%[htbp]
    \small\centering
    \begin{tabular}{lccc}
    \toprule
          Model & UPOS & LAS & NER\\
    \midrule
   Baseline & \textbf{89.97} & 67.09 & \bf  50.12 \\
   UyghurBERT   & 87.39  & \textbf{77.33} & 41.42 \\
   \mbert  &  76.98 & 72.26 & 24.32 \\
   \mbertmlm &  88.41 & 48.91 & 34.66 \\
    \bottomrule
    \end{tabular}
    \caption{Uyghur is a hard language. The non-contextual baseline outperforms all \mbert variants on POS tagging, and the UyghurBERT is best for DEP.\iffalse \hl{see comment table 10 -ds}\fi}
    \label{tab:uighur}
\end{table}

==> figs/single_lang_tables/wolof.tex <==

\begin{table}[htbp]
    \centering\small
    \begin{tabular}{lccc}
    \toprule
        Model & UPOS & LAS \\
    \midrule
        Baseline & 94.09 & 77.05 \\ 
        WolofBERT & 88.41 & 52.8 \\
        \mbert & 92.85 & 73.26\\
        \mbert+MLM & \textbf{95.22} & \textbf{77.91}\\
    \bottomrule
    \end{tabular}
    \caption{Wolof falls into the Intermediate category. \mlmtuning enables \mbert to match or outperform strong non-contextual baselines}%the results for POS tagging fall into the ``Intermediate'' pattern, but for DEP fall in the ``easy'' unseen languages pattern.}
    \label{tab:wolof}
\end{table}

==> figs/transliterartion_with_controlled_exp_2.tex <==

\begin{table*}[t]
    \centering\footnotesize
    \scalebox{0.9}{ % w
    \begin{tabular}{c|ccc||c|c}
    \toprule
         Model & \multicolumn{1}{c}{POS} & \multicolumn{1}{c}{LAS} & \multicolumn{1}{c}{NER} & Model & NER \\
         
    \midrule
    \multicolumn{4}{c||}{Uyghur (Arabic$\rightarrow$Latin)} & \multicolumn{2}{c}{Sorani (Arabic$\rightarrow$Latin)}
\\
    UyghurBERT & 87.4$\rightarrow$86.2 & 57.3$\rightarrow$54.6 & 41.4$\rightarrow$41.7 
    & SoraniBERT & 80.6$\rightarrow$78.9 

    \\
    
    \mbert & 77.0$\rightarrow$87.9 & 45.7$\rightarrow$65.0 & 24.3$\rightarrow$35.7 &
    \mbert & 70.5$\rightarrow$77.8\\
    
    \mbertmlm & 77.3$\rightarrow$\textbf{89.8} & 48.9$\rightarrow$\textbf{66.8} & 34.7$\rightarrow$\textbf{55.2} & 
    \mbertmlm & 75.6$\rightarrow$\textbf{82.7}\\
    
    
    \midrule
    \multicolumn{4}{c||}{Buryat (Cyrillic$\rightarrow$Latin)} & \multicolumn{2}{c}{Meadow Mari (Cyrillic$\rightarrow$Latin)} \\
    BuryatBERT & 75.8$\rightarrow$75.8 & 31.4$\rightarrow$31.4 & -- & MariBERT & 44.0$\rightarrow$45.5\\
    \mbert & 83.9$\rightarrow$81.6 & 50.3$\rightarrow$45.8 & -- & \mbert & 55.2$\rightarrow$58.2\\
    \mbertmlm & \textbf{86.5}$\rightarrow$84.6 & \textbf{52.9}$\rightarrow$51.9 & -- & \mbertmlm & 57.6$\rightarrow$\textbf{65.9}\\
    \midrule
    
    \multicolumn{4}{c||}{Erzya (Cyrillic$\rightarrow$Latin)} & \multicolumn{2}{c}{Mingrelian (Georgian$\rightarrow$Latin)} \\
    ErzyaBERT & 84.4$\rightarrow$84.5 & 47.8$\rightarrow$47.8  & -- & MingrelianBERT & 42.0$\rightarrow$42.2\\
    \mbert & 89.3$\rightarrow$88.2 & 61.2$\rightarrow$58.3 & -- & \mbert & 53.6$\rightarrow$41.8\\
    \mbertmlm & \textbf{91.2}$\rightarrow$90.5 & \textbf{66.6}$\rightarrow$65.5 & -- & \mbertmlm & \textbf{68.4}$\rightarrow$62.6\\
    \hdashline
     & \multicolumn{2}{c}{Arabic (Arabic$\rightarrow$Latin)}\\
    \mbert & xx.x $\rightarrow$ 94.9 & xx.x $\rightarrow$ 78.8  & xx.x $\rightarrow$ xx.x  \\
    & \multicolumn{2}{c}{Russian (Cyrillic$\rightarrow$Latin)}\\
    \mbert & 98.14 $\rightarrow$ 96.01 & xx.x $\rightarrow$84.5 & xx.x \\
    & \multicolumn{2}{c}{Japanese (Japanese$\rightarrow$Latin)}\\
    \mbert & 97.38$\rightarrow$95.66 & 88.5$\rightarrow$ 86.93 &   \\
    
    \bottomrule
    \end{tabular}
}
    \caption{Transliterating low-resource languages into the Latin script leads to significant improvements in languages like Uyghur, Sorani, and Meadow Mari. For languages like Erzya and Buryat transliteration does not significantly influence results, while it does not help for Mingrelian. In all cases, \mbertmlm is the best approach.\iffalse \hl{THis caption should be the comment of that table in the core text or appears distinclty from the table description -ds. }\fi}
    \label{tab:translit}

\end{table*}



==> figs/transliteration_as_adaptation.tex <==

\begin{table*}[ht]
\small\centering
\resizebox{\linewidth}{!}{
\begin{tabu}{ l  c  c  c@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c   c c@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c   c c}%@{\hspace{0.35cm}}  @{\hspace{0.35cm}} c  c }
	\toprule
	& \multicolumn{3}{c @{\hspace{0.5cm}}}{\textsc{UPOS}} & \multicolumn{3}{c @{\hspace{0.7cm}}}{\textsc{LAS}} & \multicolumn{3}{c @{\hspace{0.7cm}}}{\textsc{NER}} & %\multicolumn{3}{c @{\hspace{0.35cm}}}{\textsc{ParTUT}} \\
	\cmidrule(l{2pt}r{0.4cm}){2-4}\cmidrule(l{-0.2cm}r{0.4cm}){5-7}\cmidrule(l{-0.2cm}r{0.4cm}){8-10}%\cmidrule(l{-0.2cm}r{2pt}){8-9}
	\multirow{-2}{*}[1pt]{Model} & 
	\textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm & \textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm &
	\textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm &
	%\multirow{-2}{*}[1pt]{}
	%& \textsc{\mbert}   &\textsc{\mbertmlm} & \monomlm & Baseline 
	%\multirow{-2}{*}[1pt]{} 
	%& \textsc{\mbert}     &\textsc{\mbertmlm} & \monomlm & Baseline 
	\\
	%\textit{In-Languages translit Arabic as control exp.(?)} \\

	
	
	\midrule
	   

	Uyghur &  76.98 & 77.33 & 87.39 & 45.47 & 48.91 & 57.29 & 24.32 & 34.66 & 41.42\\
	Uyghur \textsc{Latin} & 87.92 & \bf 89.81 & 86.19 & 64.98 & \bf 66.81 &54.58 &35.07&\bf 55.23& 41.68 \\
%	Uyghur \permute & &&&36.41\\

	%x & x & x & x &\\
	\midrule
    %\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
    Sorani & 
	% POS
	- & - & - & - & - & - & 70.45 & 75.56 & 80.58 \\
	Sorani \textsc{Latin} & - & - & - & - & - & - & 77.78 & \bf 82.72 & 78.91 \\
	% 79.31
	
	%Sorani +\translit (on translit)& - & - & - & - & - & - & \bf  & x & 79.31 \\
    %\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
	%Sorani +\translit & 
	% POS - & - & - & - & - & - & \bf 81.21 & x & x \\
	\midrule
	%\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
    Mingrelian & 
	% POS
	- & - & - & - & - & - &  53.64 &\bf68.40 & 42.01 \\
	Mingrelian \textsc{Latin} & 
	% POS
	- & - & - & - & - & - & 41.76 & 62.58 & 42.22 \\    
	%Mingrelian + \translit (on translit) & - & - & - & - & - & - & 48.74 & x & x \\
	%Mingrelian + \translit (on native  ) & - & - & - & - & - & - & 53.93 & x & x \\
	\midrule
	%\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
    Meadow Mari & 
	% POS
	- & - & - & - & - & - &  55.19 & 57.62 & 43.97 \\
	Meadow Mari \textsc{Latin} & 
	% POS
	- & - & - & - & - & - & 58.20 & \bf 65.89 & 45.45 \\
	\midrule
	Buryat  & 
	% POS
	83.88 & \bf 86.45 & 75.77 & 50.34 & \bf 52.95 & 31.35 &  - & - & - \\
	Buryat \textsc{Latin}& 
	% POS
	81.60 & \bf 84.56 & 75.77 & 45.76 & \bf 51.88 & 31.35 & - & - & - \\
	\midrule
	Erzya   & 
	% POS
	89.27 &  \bf 91.19 & 84.41 &61.21 & \bf 66.56  & 47.80 &  - & - & - \\
	Erzya  \textsc{Latin} & 
	% POS
	88.21 & 90.53 & 84.52& 58.33 & \bf 65.50 & 47.80  & - & - & - \\
	\midrule
	Livi  & \bf 82.98 &  \bf 85.46 & 70.86 &  36.25&\bf 42.28 & 30.80  & - & - & -\\
	Livi \textsc{Cyrillic}  & 74.36 & \bf 85.91 &70.67 & 38.52& \bf 41.53  & 30.22 & - & -& -\\
	
	
	
	
    %Meadow Mari + \translit (eval translit) &  - & - & - & - & - & - & \bf 57.32 & x & x \\
  %  \tabucline[\hbox {$\scriptstyle \cdot$}]{-}
   % Meadow Mari + \translit (eval native) &  - & - & - & - & - & - & \bf 60.90 & x & x \\
%	Sorani \permute & 
	% POS
%	- & - & - & - & - & - & x & x & x \\

	%\textit{Control experiment}\\

	%Wolof &  92.85 & 95.22 &x & 73.26&77.91& x&  - & - & - \\
	%Wolof Cyrillic & 92.67  &95.19&x   & 72.42 & 78.24&x &  - & - & - \\
	 % Wolof with mbert+mlm cyr on wolof latin UPOS: 93.83, LAS; 75.68
	 
	%\tabucline[\hbox {$\scriptstyle \cdot$}]{-}
	

	%\camembert (fine-tuned)                           & \textbf{98.18}    & \textbf{92.57}    & \underline{99.29}          & \textbf{94.20}    & 96.99             & 81.37             & \textbf{97.65}    & \textbf{93.43}             \\ % 10125734 : POS best seed PARSING gsd 10126431 PARSING other : 10126429
	%UDPipe Future \mbox{+ \camembert} (embeddings)    & 97.96             & 90.57             & 99.25          & \underline{93.89}             & \underline{97.09}             & \textbf{81.81}             & 97.50             & 92.32             \\
	\bottomrule
\end{tabu}
}
\caption{\textbf{POS}, \textbf{Dependency Parsing} and \textbf{NER} scores obersving the impact of the script on \mbert, \mbertmlm  and \monomlm. \textsc{Latin} means training and evaluation on data transliterated in the Latin script %(for Uyghur, we do "turkification") 
}%
\label{tab:transliteration}
\end{table*}

==> figs/transliteration_with_controlled.tex <==

\begin{table*}[t]
    \centering\footnotesize
    \scalebox{0.8}{ % w
    \begin{tabular}{c|ccc||c|c||c|ccc}
    \toprule
         Model & \multicolumn{1}{c}{POS} & \multicolumn{1}{c}{LAS} & \multicolumn{1}{c}{NER} & Model & NER & Model  & POS & LAS & NER \\
         
    \midrule
    \multicolumn{4}{c||}{Uyghur (Arabic$\rightarrow$Latin)} & \multicolumn{2}{c}{Sorani (Arabic$\rightarrow$Latin)}
    & \multicolumn{2}{c}{Arabic (Arabic$\rightarrow$Latin)}
    \\
    UyghurBERT & 87.4$\rightarrow$86.2 & 57.3$\rightarrow$54.6 & 41.4$\rightarrow$41.7 
    & SoraniBERT & 80.6$\rightarrow$78.9 
    & \mbert & xx.x $\rightarrow$ 94.9 & xx.x $\rightarrow$ 78.8  & $\rightarrow$ 78.8  
    \\
    
    \mbert & 77.0$\rightarrow$87.9 & 45.7$\rightarrow$65.0 & 24.3$\rightarrow$35.7 &
    \mbert & 70.5$\rightarrow$77.8\\
    
    \mbertmlm & 77.3$\rightarrow$\textbf{89.8} & 48.9$\rightarrow$\textbf{66.8} & 34.7$\rightarrow$\textbf{55.2} & 
    \mbertmlm & 75.6$\rightarrow$\textbf{82.7}\\
    
    
    \midrule
    \multicolumn{4}{c||}{Buryat (Cyrillic$\rightarrow$Latin)} & \multicolumn{2}{c}{Meadow Mari (Cyrillic$\rightarrow$Latin)} \\
    BuryatBERT & 75.8$\rightarrow$75.8 & 31.4$\rightarrow$31.4 & -- & MariBERT & 44.0$\rightarrow$45.5\\
    \mbert & 83.9$\rightarrow$81.6 & 50.3$\rightarrow$45.8 & -- & \mbert & 55.2$\rightarrow$58.2\\
    \mbertmlm & \textbf{86.5}$\rightarrow$84.6 & \textbf{52.9}$\rightarrow$51.9 & -- & \mbertmlm & 57.6$\rightarrow$\textbf{65.9}\\
    \midrule
    
    \multicolumn{4}{c||}{Erzya (Cyrillic$\rightarrow$Latin)} & \multicolumn{2}{c}{Mingrelian (Georgian$\rightarrow$Latin)} \\
    ErzyaBERT & 84.4$\rightarrow$84.5 & 47.8$\rightarrow$47.8  & -- & MingrelianBERT & 42.0$\rightarrow$42.2\\
    \mbert & 89.3$\rightarrow$88.2 & 61.2$\rightarrow$58.3 & -- & \mbert & 53.6$\rightarrow$41.8\\
    \mbertmlm & \textbf{91.2}$\rightarrow$90.5 & \textbf{66.6}$\rightarrow$65.5 & -- & \mbertmlm & \textbf{68.4}$\rightarrow$62.6\\
    \bottomrule
    \end{tabular}
}
    \caption{Transliterating low-resource languages into the Latin script leads to significant improvements in languages like Uyghur, Sorani, and Meadow Mari. For languages like Erzya and Buryat transliteration does not significantly influence results, while it does not help for Mingrelian. In all cases, \mbertmlm is the best approach.\iffalse \hl{THis caption should be the comment of that table in the core text or appears distinclty from the table description -ds. }\fi}
    \label{tab:translit}

\end{table*}



==> highresource.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{cccc|cccc}
    \toprule
        Language & Treebank & Representation & Task-Tuning & UPOS & FEATS & UAS & LAS\\
    \midrule
    \multirow{3}{*}{Dutch} & \multirow{3}{*}{Lassy Small} & BERTje & mono & 96.32 & 96.45 & 91.65 & 88.32 \\ 
    & & mBERT & mono & 96.10 & \textbf{96.71} & 92.02 & 88.79\\ 
    & & mBERT & all & \textbf{96.70} & 96.57 & \textbf{94.34} & \textbf{91.22}\\
    \midrule
    \multirow{12}{*}{German} & \multirow{3}{*}{GSD} & german-BERT & mono & 93.85 & 72.26 & 87.28 & 82.63 \\
        & & mBERT & mono & 93.59 & 70.77 & 86.30 & 81.28 \\ 
        & & mBERT & all & \bf 94.55 & \bf 90.54 & \bf 88.40 & {\bf 84.03} \\ \cmidrule{3-8}
    & \multirow{3}{*}{HDT} & german-BERT & mono & \bf 98.46 & \bf 93.24 & \bf 97.35 & {\bf 96.29} \\
        & & mBERT & mono & \bf 98.45 & 93.07 & 97.07 & 95.83 \\
        & & mBERT & all & 91.10 & 33.14 & 90.50 & \hl{85.21} \\ \cmidrule{3-8}
    & \multirow{3}{*}{LIT} & german-BERT & mono & \bf 93.69 & 32.41 & \bf 86.23 & {\bf 79.76} \\
        & & mBERT & mono &\bf  93.77 & 31.10 & 85.84 & 79.16 \\
        & & mBERT & all & 92.08 & \bf 37.88 & 84.89 & \hl{79.56} \\ \cmidrule{3-8}
    & \multirow{3}{*}{PUD} & german-BERT & mono & 90.29 & 29.00 & 88.57 & 83.29 \\
        & & mBERT & mono & \bf 90.76 & 29.24 & 88.29 & 82.72 \\
        & & mBERT & all & 89.54 & \bf 30.71 & \bf 89.61 & \hl{\bf 84.28} \\
    \midrule
    \multirow{12}{*}{Japanese} & \multirow{3}{*}{bccwj} & 
        jap-BERT & mono & \bf 33.37 & \bf 98.8 & \bf 28.34 &\bf  17.66 \\ 
        & & mBERT & mono & \bf 33.33 & \bf 98.8 & \bf 28.34 &\bf  17.68 \\ 
        & & mBERT & all & 21.18 & 91.50 & 15.64 & \hl{6.58}\\ \cmidrule{3-8}
     & \multirow{3}{*}{GSD} & jap-BERT & mono & \bf 97.18 & 99.97 & 94.18 & \bf 91.97 \\ 
        & &mBERT & mono & 96.76 & 99.96 & 93.78 & 91.37 \\ 
        & &mBERT & all & 96.67 & 99.97 & \bf 94.58 & \hl{91.78} \\ \cmidrule{3-8}
    & \multirow{3}{*}{modern} & jap-BERT & mono & 74.72 & 96.57 & \bf 76.65 & \bf 54.98 \\ 
        & & mBERT & mono & 72.89 & \bf 96.59 & 74.81 & 53.79 \\ 
        & & mBERT & all & \bf 74.94 & 96.16 & 74.96 & \hl{53.87} \\ \cmidrule{3-8}
    & \multirow{3}{*}{PUD} & jap-BERT & mono & \bf 97.41 & 99.95 & 93.79 & 92.09 \\ 
        & & mBERT & Japanese & 97.35 & 99.97 & 93.98 & 92.34 \\ 
        & & mBERT & all & 97.13 & 99.98 &\bf  95.18 & \hl{\bf 92.95}\\
    \midrule
    \multirow{9}{*}{Finnish} & \multirow{3}{*}{FTB} & finBERT & mono & \bf 96.27 & \bf 93.38 & \bf 89.43 & \bf 85.95 \\
        & & mBERT & mono & 93.06 & 89.85 & 83.12 & 77.48 \\ 
        & & mBERT & all & 90.97 & 90.56 & 86.07 & \hl{80.92} \\ \cmidrule{3-8}
     & \multirow{3}{*}{TDT} & finBERT & mono & \bf 96.34 & \bf 92.88 & \bf 88.37 & \bf 84.71 \\
        & & mBERT & Finnish & 95.04 & 90.27 & 83.59 & 78.91 \\ 
        & & mBERT & all & 94.33 & 90.47 & 86.32 & \hl{81.78} \\ \cmidrule{3-8}
      & \multirow{3}{*}{PUD} & finBERT & mono & \bf 97.47 & \bf 95.67 & \bf 90.81 & {\bf 88.19} \\
        & & mBERT & mono & 96.80 & 93.84 & 87.04 & 83.45 \\ 
        & & mBERT & all & 96.77 & 93.98 & 89.60 & \hl{86.21} \\        
    \bottomrule
    \end{tabular}
    \caption{High-resource languages}
    \label{tab:high}
\end{table*}


==> lowwith.tex <==
\an{TODO: lowwith}

==> lowwithout.tex <==
\an{TODO: lowwithout}

==> midwith.tex <==
\begin{table*}[t]
    \centering\small
    \begin{tabular}{cccc|cccc}
    \toprule
        Language & Treebank & Representation & Task-Tuning & UPOS & FEATS & UAS & LAS\\
    \midrule
    \multirow{3}{*}{Naija} & \multirow{3}{*}{} & mBERT & mono & \bf 89.27  & - & \bf 81.01 & \bf 71.55 \\
        & & XLM-R & mono & 87.75  & - & 79.48 & 69.41 \\
        & & BERT & mono & \bf 89.46  & - & 80.96 & 71.40~ \\
    \hdashline
    & & mBERT & En (ewt) & 78.78  & - & \bf 76.04 & \bf 62.62 \\
    & & XLM-R & En (ewt) & \bf 82.73  & - & 69.50 & 55.92 \\
    & & BERT & En (ewt) & 77.72  & - & \bf 75.99 & 62.11 \\
    \midrule
    %\multirow{6}{*}{Maltese} & \multirow{6}{*}{} &  maltBERT oscar & mono & 91.08 & - & 68.66&  61.57   \\
    \multirow{6}{*}{Maltese} & \multirow{6}{*}{} &  maltBERT 100k & mono & 90.39 & - & 64.38 &  56.48  \\
     &  &  maltBERT 1M & mono & 91.05 & - & 70.13 & 62.12   \\
  &  &  maltBERT 5M & mono & 92.05 & - & 74.11 & 66.55   \\

    & & mBERT & mono & 92.04  & - & 81.60 & 74.41 \\ 
    & & mBERT MT & mono & 92.77 & \bf 100 & 81.14 & 74.59 \\ 
    & & mBERT MT +MLM (5M) & mono & \bf 93.39 & \bf 100 & 82.46 & \bf 76.31 \\
    & & mBERT & similar & xx & xx & xx & xx \\
    & & mBERT +FT (5M) & similar & xx & xx & xx & xx \\
    & & mBERT MT & all & 91.98 & 99.89 & \bf 83.07 & 75.56 \\
    
    \midrule
    \\
    \multirow{6}{*}{Narabizi} & \multirow{6}{*}{} & NarzBERT & mono & 71.35 & - & 51.55 & 41.78 \\ 
    & & CamemBERT & mono & xx & - & 66.04 & 54.10  \\
    & & mBERT & mono & \underline{81.60} & -  & \underline{67.77} & \underline{56.52} \\
    %& & mBERT +FT (50k) & mono & \bf 83.20 & - & \bf 67.82* & \bf 57.15* \\
    & & mBERT +FT (50k) & mono & \bf 84.22 & - & \bf 69.32 & \bf 57.83 \\ % 10812914
    & & XLM-R & mono & 79.74 & - & 65.17 & 53.61  \\
    & & XLM-R +FT 50k & mono & \bf 85.53 & - & 71.30 & 59.86  \\% 10812914
    \hdashline
    & & mBERT & Maltese & \bf 35.13 & - & \bf 40.04 & \bf 18.49 \\
    & & mBERT & Arabic & 16.55 & - & 28.23 & 10.95 \\
    & & mBERT & French &  33.12 & - & 38.54 & 16.12 \\
    & & Camembert & Maltese & 31.62 & - & 34.65 & 10.57 \\
    & & Camembert & French & 31.77 & - & 32.55 & 12.26 \\
    & & mBERT & all & x &x & xx & x \\
    \midrule
    
     \\
    \multirow{6}{*}{Uyghur} & \multirow{6}{*}{} 
    & UgBERT (105k) & Ug & \bf{87.39} & - & 
    \bf{70.89} & \bf{57.29} \\ 
    & & araBERT  & Ug & \underline{79.77} & - & 
    \underline{67.95} & \underline{51.67} \\ 
    & & araBERT+FT 105k  & Ug & x & - & 
    x & x \\ 
    & & mBERT & Ug & 75.76 & - & 63.61 & 45.47 \\
    & & mBERT FT 105k & Ug & 76.98 & - & 65.63 &  49.00 \\% 10813134 / unsup-tuning 10811974
    & &mBERT MT & Ug & 76.02 & 71.38 & 64.22 & 48.26 \\ 
    & &mBERT MT+ MLM FT (10K) & Ug & 76.17 & 71.22 & 64.18 & 48.67 \\
    & &mBERT MT+MLM FT (30K) & Ug & 75.76 & 71.54 & 64.30 & 48.31\\
    \hdashline
    & & XLM-R & Ug & 87.66 & - & 76.03  & 64.05 \\
    & & XLM-R FT 105k & Ug & \underline{89.49} & - & \underline{78.76}  & \underline{65.97} \\
    & & XLM-R FT Uy(50k)/Tr(50k) & Ug &  x & - & \bf  80.34  & \bf  68.14 \\
    \hdashline
    & & XLM-R FT 105k & Ug+Hu(1k) &  88.84 & - & \bf 79.34  & \bf 66.59 \\
    & & XLM-R FT 105k & Ug+Tr(1k) &  88.39 & - & 78.53  &  65.93 \\
    \hdashline
    
    \hdashline
    & & mBERT & Turkish & 37.91 & - & 17.15  & 9.53  \\
    & & XLM-R & Turkish &  77.91 & - & 53.43 & 38.87 \\
    
    \bottomrule
    \end{tabular}
    \caption{\textcolor{red}{NEW} Mid-resource languages with task training data. (monolingual BERT trained from scratch are MLM only (no next-sentence prediction) with sentence piece tokenization. 
    mBERT MT (Multitask) is Udify architecture trained on the refered treebank}
    \label{tab:midwith}
\end{table*}


==> midwithout.tex <==
\begin{table*}[t]
    \centering\small
    \begin{tabular}{cccc|cccc}
    \toprule
        Language & Treebank & Representation & Task-Tuning & UPOS & FEATS & UAS & LAS\\
    \midrule
    \multirow{6}{*}{Faroese} & \multirow{6}{*}{xx} & Faroese-BERT 285k & Scand & xx & - & 45.69 & 35.82 \\ 
    & & SwedishBERT & Scand & xx & - & 57.41 & 44.88 \\ 
    & & SwedishBERT + FT (1M) & Scand & xx & - & 65.80 & 46.82 \\
    %& & mBERT & Scand & x & - & x & x \\ 
    & & mBERT MT & Scand & 79.39 & 35.38 & 74.73 & 67.50 \\ 
    & & mBERT MT+FT (1M) & Scand & 79.37 & 35.50 & 75.28 & 67.82 \\
    & & mBERT & all & \bf 91.98 & \bf 99.89 & \bf 83.07 & \bf 75.56 \\
    \midrule
    \multirow{6}{*}{Swiss German} & \multirow{6}{*}{xx} & mono & De GSD  & \underline{64.65} & - & 45.86 & 29.97 \\ 
    & & german-BERT & De GSD & 48.72 & - & 37.71 & 23.75 \\
    & & german-BERT +FT (200K) & De GSD & xx & - & \bf  75.83 & \bf 63.57 \\ 
    & & XLM-R & De GSD & xx & - & 36.95 & 25.03 \\ 
    & & mBERT & De GSD & 62.67  & - & 52.91 & 36.15\\
    & & mBERT MT & German & 63.50 & 48.06 & 54.16 & 42.45 \\ 
    & & mBERT MT+FT (200K) & German & 64.61 & \bf 50.07 & 53.46 & 41.62 \\
    & & mBERT & all & \bf 77.46 & 35.20 & \underline{67.24} & \underline{59.26} \\
    \midrule
    \multirow{3}{*}{Amharic} & \multirow{3}{*}{xx} & Am-Bert & similar? & xx & xx & xx & xx \\
 & & mBERT & similar? & xx & xx & xx & xx \\ 
 & & mBERT & English & 10.93 & xx & 10.71 & 10.68 \\ 
  %& & XLM-R & English & \bf 49.60 & - & \bf 55.48 & \bf 22.46 \\
  & & XLM-R & English & 49.60 & - & 38.34 &  13.18 \\
  & & XLM-R FT 67k & English & \bf x & - & \bf 53.27 & \bf 21.98 \\ 
  \hdashline
  & & XLM-R & English+Am(10) & x & - & \bf 68.53 &   42.14 \\
  & & XLM-R FT 67k & English+Am(10) & x & - & \bf 68.27 &  \bf 45.47 \\
  \hdashline
  & & XLM-R & Arabic & x & - &  41.79 &  21.98 \\ 
  & & XLM-R FT 67k & Arabic & x & - &  45.07 &  16.29 \\ 


    \midrule

    
    \multirow{3}{*}{Tagalog} & \multirow{3}{*}{xx} & ta-Mbert & Indo & 44.01 & - & 49.32 & 30.14 \\
    &&IndoBERT & Indo & 38.18 & - & 29.97 &  20.55\\
    &&mBERT & Indo &  \underline{68.01} & - & \underline{62.67} & \underline{40.24}\\
    &&XLM-R & Indo & \bf 71.23 & - & \bf 84.25 & \bf 57.02\\
    \hdashline
    &&mBERT & English & 85.88* & - & 82.88 & 55.82\\
    & & XLM-R & English & \bf 87.33  & - & \bf 83.05 & \bf 57.71 \\
  
 \midrule
\multirow{7}{*}{Kurmanji} & \multirow{7}{*}{xx} & Sorani-Bert & Kurmanji(20) & 45.18 & xx & xx & xx \\ 
& & mBERT & Kurmanji(20) & 54.71 & - & 19.39 & 11.83 \\ 
\hdashline
&& Sorani-Bert & Kur+Fa(1k) & 52.56 & xx & 15.72 & 10.23 \\ 
& & XLM-R & Kur+Fa(1k) & 76.9 & - & x & x \\
& & mBERT & Kur+Fa(1k) & \bf 63.18 & - & 33.51 & 23.56 \\ 
\hdashline
& & mBERT MT & all & 60.23 & - & 19.39 & 11.83 \\




    \bottomrule
    \end{tabular}
    \caption{Mid-resource languages without task training data.}
    \label{tab:midwithout}
\end{table*}

==> name.tex <==
Transfer learning based on pretraining language models on a large amount of raw data has become a new norm to reach state-of-the-art performance in NLP. Still, it remains unclear how this approach should be applied for unseen languages that are not covered by any available large-scale multilingual language model and for which only a small amount of raw data is generally available. In this work, by comparing multilingual and monolingual models, we show that such models behave in multiple ways on unseen languages. Some languages greatly benefit from transfer learning  and behave similarly to closely related high resource languages whereas others apparently do not. Focusing on the latter, 
we show that this failure to transfer is largely related to the impact of the script used to write such languages. Transliterating those languages improves very significantly the ability of large-scale multilingual language models on downstream tasks.

==> original_section4_2-4.3+5.tex <==
\subsection{Intermediate}
The second type of languages (which we dub ``Intermediate'') are generally harder to process for pretrained MLMs out-of-the-box. In particular, pretrained multilingual language models are typically outperformed by a non-contextual strong baselines. Still, \mlmtuning has an important impact and leads to usable state-of-the-art models. 

A good example of such an intermediate language is Maltese, a member of the Semitic language but using the Latin script, Maltese has not been seen by \mbert. Other Semitic languages though, namely Arabic and Hebrew, have been included in the pre-training languages. \draftreplace{The results on Maltese are outlined in Table~\ref{tab:maltese}, where it is clear that the non-contextual baseline outperforms \mbert.}{As seen in Table~\ref{tab:intermediate}, the non-contextual baseline outperforms \mbert.} Additionally, a monolingual MLM trained on only 50K  sentences matches \mbert performance for both NER and POS tagging. However, the best results are reached with \mlmtuning: the proper use of monolingual data and the advantage of similarity to other pre-training languages render Maltese a {\em tackle-able} language \draftreplace{by outperforming our strong non-contextual baseline.}{as show by the gain of performance over our strong non-contextual baselines.} 





%\input{figs/single_lang_tables/maltese}
%\an{
Our Maltese dependency parsing results are in line with those of~\citet{chau2020parsing}, who also showed that \mlmtuning leads to significant improvements. They also additionally showed that a small vocabulary transformation allowed finetuning to be even more effective and gain 0.8 LAS points more. We further discuss the vocabulary adaptation technique of~\cite{chau2020parsing} in Section~\ref{sec:discussion}.
%}


We consider Narabizi \citep{seddah-etal-2020-building}, an Arabic dialect spoken in North-Africa written in the Latin script and code-mixed with French, to fall in the same ``Intermediate'' category, because it follows the same pattern. \draftremove{Our results in Narabizi are listed in Table~\ref{tab:narabizi}.} 
For both POS tagging and parsing, the multilingual models outperform the monolingual NarabiziBERT. In addition, \mlmtuning leads to significant improvements over the non-language-tuned \mbert baseline, also outperforming the non-contextual dependency parsing baseline.

%\input{figs/single_lang_tables/narabizi}

We also categorize Bambara, a Niger-Congo Bantu language spoken in Mali and surrounding countries, as Intermediate, relying mostly on the POS tagging results which follow similar patterns as Maltese and Narabizi\draftremove{(see  Table~\ref{tab:bambara})}. We note that the BambaraBERT that we trained achieves notably poor performance compared to the non-conctextual baseline, a fact we attribute to the extremely low amount of available data (1000 sentences only). We also note that the non-contextual baseline is the best performing model for dependency parsing, which could also potentially classify Bambara as a ``Hard" language instead.

%\input{figs/single_lang_tables/bambara}

Our results in Wolof follow the same pattern. The non-contextual baseline achieves a 44.1 F1 score. A monolingual WolofBERT with an LAS score of 45.2 outperforms \mbert (42.3). However, \mlmtuning achieves the highest F1-score of 47.9.

%Our results in Sindhi follow the same pattern. The non-contextual baseline achieves a 44.1 F1 score. A monolingual SindhiBERT with an F1-score of 45.2 outperforms \mbert (42.3). However, \mlmtuning achieves the highest F1-score of 47.9. Similarly, for Wolof \mbert outperforms the non-contextual baseline only after \mlmtuning. 

%\input{figs/single_lang_tables/wolof}







\subsection{Hard}

%\input{figs/single_lang_tables/uyghur}
\input{figs/hard_summary}

The last category of the hard unseen language is perhaps the most interesting one, as these languages are very hard to process. \draftreplace{All available large-scale language models are}{\mbert is} outperformed by non-contextual baselines as well as by monolingual language models trained from scratch on the available raw data. At the same time, \mlmtuning on the available raw data has a minimal impact on performance. 


Uyghur, a Turkic language with about 10-15 million speakers in central Asia, is a prime example of a hard language for current models. In our experiments, outlined in Table~\ref{tab:hard_summary}, the non-contextual baseline outperforms all contextual variants, both monolingual and multilingual, in all the tasks with up to 20 points difference compared to \mbert for parsing. Additionally, the monolingual UyghurBert trained on only 105K sentences outperforms \mbert even after \mlmtuning. Finally, 
%The non-contextual baseline achieves the scores in all the three tasks with up to 20 points difference compared to \mbert for parsing. 

%The monolingual UyghurBert achieves the best dependency parsing results with a LAS of 77, more than 5 points higher than \mbert, with similar trends for NER. Uyghur is also the only case %where \mbert 
%for which \mlmtuning does not improve over the unadapted \mbert on dependency parsing.



We attribute this discrepancy to script differences: Uyghur uses the Perso-Arabic script, when the other Turkic languages that were part of \mbert pre-training use either the Latin (e.g. Turkish) or the Cyrillic script (e.g. Kazakh). 
%\an{Regarding presentation: I would *probably* present the results in smaller tables instead of big Tables with all results. Although the bigger tables allow for easier comparisons}
%\BM{agree , with adding a summary table in introduction as we discussed}


Sorani Kurdish (also known as Central Kurdish) is a similarly hard language, mainly spoken in Iraqi Kurdistan by around 8 million speakers, which uses the Sorani alphabet, a variant of the Arabic script. We can solely evaluate on the NER task, \draftreplace{where the non-contextual baseline is the best model, achieving a 81.3 F1-score. The SoraniBert that we trained reaches 80.6 F1-score, while \mbert gets 70.4 F1-score.}{where the non-contextual baseline and the monolingual SoraniBERT perform similarly around 80.5 F1 outperforming significantly \mbert which only reach 70.4 in F1.} \mlmtuning on 380K sentences of Sorani texts improves \mbert performance to 75.6 F1-score, but it is still lagging behind the baseline. Our results in Sindhi follow the same pattern. The non-contextual baseline achieves a 51.4 F1 score outperforming with a large margin contextual language models. .% A monolingual SindhiBERT with an F1-score of 45.2 outperforms \mbert (42.3).

\iffalse
\begin{figure}[t]
\centering
\includegraphics[width=8cm]{pic/script-illustrate.png}
\caption{An illustration of the pretraining distributions and an unseen language distribution in the case of the Turkic Language Family. Uyghur is unseen but related to Turkish which \mbert has been pretrained on. Uyghur is written in the Arabic script while Turkish is written in the Latin Script making it a tough challenge for \mbert}
\end{figure}
\fi 

\input{figs/transliteration_final}
%\input{figs/transliteration_with_controlled}
%\input{figs/transliterartion_with_controlled_exp_2}

\section{Tackling Hard Languages with Multilingual Language Models}
%cf. Table \ref{tab:transliteration}

Our ``intermediate" language results provide initial supporting evidence for our argument on the importance of having pretrained LMs on languages with similar scripts, even for generally high-resource language families.
%% ICIDJAME
\textcolor{red}{We first focus on Uralic languages. Finnish, Estonian, and Hungarian are high-resource representatives of this language family that are typically included in multilingual LMs, also having task-tuning data available in large quantities. However, for several smaller Uralic languages, task-tuning data are generally very scarce.}

\textcolor{red}{Table~\ref{tab:intermediate} reported the performance for two low-resource Uralic languages, namely Livvi and Erzya using 8-fold cross-validation, with each run only using around 700 training instances. \draftreplace{For both Livvi and Erzya, the multilingual model along with \mlmtuning achieves the best performance, outperforming the non-contextual baseline by more than 1.5 point for parsing and POS tagging. Additionally, we observe a}{Note the} striking difference between the parsing performance (LAS) of \mbert on Livvi (which uses the Latin script) and on Erzya that uses the Cyrillic script. This suggests that the script could be playing a critical role when  transferring to those languages.
}

%As we have already alluded to, our hypothesis is that the script is a key element for \draftreplace{pretrained multilingual}{language} models to correctly process unseen languages. 

To verify our hypothesis on the importance of script, we assess the ability of \mbert to process an unseen language after transliterating it to another script. We focus our experiments on six languages belonging to four language families: Erzya, Bruyat and Meadow Mari (Uralic), Sorani Kurdish (Iranian, Indo-European), Uyghur (Turkic) and Mingrelian (Kartvelian). We apply the following transliteration: 
\begin{itemize}
    %%% benjamin, appelle moi si t'as 5Mn. Y a un truc que je ne comprends pas du tout
    \item Erzya/Buryat/Mari: Cyrillic $\xrightarrow{}$ Latin Script % ^^^^^^
    \item Uyghur: Arabic Script
    $\xrightarrow{}$ Latin Script
    \item Sorani: Arabic Script $\xrightarrow{}$ Latin Script
    \item Mingrelian: Georgian Script $\xrightarrow{}$ Latin Script
\end{itemize}

\input{benoit_translit}

\subsection{Transfer via Transliteration}%% added by djame
\label{sec:translit}
%transliterate them to the Latin script. 
We train \mbert with \mlmtuning and \tasktuning as well as monolingual BERT model trained from scratch on the transliterated data. %As a control experiment, we also train a monolingual BERT Model from scratch on the transliterated data of each language. 
\draftadd{We also run controlled experiments  on high-resource languages written in the Latin script on which \mbert was pretrained on, namely Arabic, Japanese and Russian (reported in Table~\ref{tab:controlled_exp}).} %For all the three tasks,  transliterating those languages to the latin script leads to a sharp drop in performance of \mbert.} 

%% table results
%\input{translit.tex}


Our results with and without transliteration are listed in Table~\ref{tab:translit}.
Transliteration for Sorani and Uyghur has a noticeable positive impact. For instance, transliterating Uyghur to Latin leads to an improvement of 16 points in parsing and 20 points in NER. For one of the low-resource Uralic languages, Meadow Mari, we observe an 8 F1-score points improvement on NER, while for other Uralic languages like Erzya the effect of transliteration is very minor.\footnote{We got similar results for Livvi (not shown in Table~\ref{tab:translit}).} 
The only case where transliterating to the Latin script leads to a drop in performance for \mbert and \mbertmlm is Mingrelian. 

 


We interpret our results as follows. When running \mlmtuning and \tasktuning, \mbert associates the target unseen language to a set of similar languages seen during pretraining based on the script. In consequence, \mbert is not able to associate a language to its related language if they are not written in the same script.  For instance, transliterating Uyghur enables \mbert to match it to Turkish, a language which accounts for a sizeable portion of \mbert pretraining. In the case of Mingrelian, transliteration has the opposite effect: transliterating Mingrelian in Latin is harming the performance as \mbert is not able to associate it to Georgian which is seen during pre-training and uses the Georgian script.

%\draftadd{%To support further our interpretation and confirm that what we are observing is not specific to languages transliterated to the Latin script 
This is further supported by our experiments  on high resource languages. When transliterating pretrained languages such as Arabic, Russian or Japanese, \mbert is not able to compete with the performance reached when using the script seen during pretraining. Transliterating the Arabic script and the Cyrillic script to Latin does not automatically improve \mbert performance as it does for Sorani, Uyghur and Meadow Mari. For instance, transliterating Arabic to the Latin script leads to a drop in performance of 1.5, 4.1 and 6.9 points for POS tagging, parsing and NER respectively.\footnote{Details and complete results on these controlled experiments can be found in Appendix~\ref{sec:controlled}.}%Indeed, transliterating Arabic and Russian to the Latin script leads to significant performance drop for our three downstream tasks.}

Our findings are generally in line with previous work. Transliteration to English specifically~\cite{lin-etal-2016-leveraging,durrani-etal-2014-integrating} and named entity transliteration \cite{kundu-etal-2018-deep,grundkiewicz-heafield-2018-neural} has been proven useful for cross-lingual transfer in tasks like NER, entity linking~\cite{rijhwani2019zero}, morphological inflection~\cite{murikinati-etal-2020-transliteration}, and Machine Translation~\cite{amrhein-sennrich-2020-romanization}.

The transliteration approach provides a viable path for rendering large pretrained models like \mbert useful for all languages of the world. Indeed, as reported in Table~\ref{tab:translit}, transliterating both Uyghur and Sorani leads to matching or outperforming the performance of non-contextual strong baselines and deliver usable models (e.g. +12.5 POS accuracy in Uyghur).\draftnote{give some numbers or a delta in relative performance -ds} %bm{confirm for NER} 



==> script.tex <==


\begin{table*}[ht!]
\footnotesize\centering
\scalebox{0.92}{ % was .7775
\begin{tabular}{lllrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
      \textit{Pretraining}&\textit{Task-tuning}&\textit{Eval}&\textsc{POS}&\textsc{LAS}&\textsc{NER} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 
%\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\

%10857697,10857698 robert-ug .
% "10858198", "10858195" xlmr-ug ... 
% 10858382, 10858383, 10858502 

%\hdashline
XLM-R &  El & El & 96.77&  89.63&&
XLM-R &  El+El Translit & El & \bf 96.97 &  \bf 90.68&&
XLM-R &  El+El Permute & El &96.58 &  90.06&&
\hline
XLM-R &  Ru & Ru & 97.24&84.53&&
XLM-R &  Ru+Ru Translit & Ru & \bf 97.39 & 85.26 &&
XLM-R &  Ru+Ru Permute & Ru &97.17 & \bf 85.55 &&
\hline
XLM-R &  Ja & Ja & 96.51 &91.64&&
XLM-R &  Ja+Ja Transl & Ja &96.48&\bf 92.06&&
XLM-R &  Ja+Ja Perm & Ja &96.45&91.79&&
\hdashline
XLM-R &  Ja Perm & Ja Perm&&88.58&&
XLM-R &  Ja Translit & Ja Translit&&82.21&&
\hline
XLM-R &  Ar & Ar & 96.13 &83.08&&
XLM-R &  Ar+Ar Translit & Ar & 96.32 &83.57&&
XLM-R &  Ar+Ar Perm & Ar & \bf 96.37 &\bf 83.80&&

%XLM-R & Mt + Ar + it & Mt+Mt shifted & Mt & &\bf  84.72&&

%XLM-R & Mt + Ar + it & Mt+Mt translit(ar)  & Mt & &\bf  &&

%\hdashline
%XLM-R & Mt + Mt translit & Mt+Mt translit & Mt &&83.46&&

\midrule

\multicolumn{1}{c}{\textit{Baselines}}&&\\
\hline

\textsc{udpipe 2.0} &&El & El& & \\
\textsc{udify} &&All &  El&   &  \\

%\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
%\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\
\bottomrule
\end{tabular}
}
%}
\caption{Does script matter ? 
}
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
\label{tab:translit}
\end{table*}


==> translit.tex <==


\begin{table*}[ht!]
\footnotesize\centering
\scalebox{0.92}{ % was .7775
\begin{tabular}{llllrrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
      \textit{Pretraining}&\textit{MLM-tuning}&\textit{Task-tuning}&\textit{Eval}&\textsc{POS}&\textsc{LAS}&\textsc{NER} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 
%\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\

%10857697,10857698 robert-ug .
% "10858198", "10858195" xlmr-ug ... 
% 10858382, 10858383, 10858502 
Ug (100k) & - & Ug & Ug & 87.39 & 57.29 & 44.98&

Ug+Ug translit & - & Ug & Ug &  87.06 & 57.59 &43.60~&
Ug+Ug translit & - & Ug+Ug Translit & Ug &    87.45 & 59.13 &43.39&
% Benoit family/script experiments 

Ug + Tr + Az + Kk  & - & Ug & Ug & 87.48 &57.52 &&
Ug + En  & - & Ug & Ug & 87.50 &57.92 &&

\hdashline
Ug + Tr + Az + Kk Translit & - & Ug Translit & Ug Translit &  82.74 & 42.23&32.17&

\hline
XLM-R & - & Ug & Ug &  86.71& 65.30 &<5&
XLM-R & - & Ug+Ug Translit & Ug & 87.12  &65.65&<5&
XLM-R & Ug  & Ug & Ug &  88.83& 65.97 &47.84&
XLM-R & Ug  & Ug+Ug Translit & Ug &  89.01& 66.46 &53.12&

XLM-R &Ug + Ug Translit  & Ug & Ug & \bf 90.49  &\underline{69.32}&\underline{60.15}&
XLM-R & Ug + Ug Translit &  Ug+Ug Translit & Ug & \underline{90.13} &\bf 70.24&\bf 63.54&


XLM-R & Ug+Tr+Az+Kk & Ug & Ug & 89.57 &68.78&to run&
XLM-R & Ug+En & Ug & Ug & 90.07 &68.61&59.70&

XLM-R & \textsc{select} & Ug & Ug & \bf 90.64 & 68.59 & 55.50&
\hdashline
XLM-R & - & Ug-Translit & Ug-Translit & 84.13 & 65.12 &<5&

XLM-R & Ug+Ug Translit  & Ug-Translit & Ug-Translit & 89.77 &67.29&\bf 56.70&
XLM-R & Ug+Tr+Az+Kk Translit & Ug Translit & Ug Translit &  89.67 &67.72&50.69&
XLM-R & Ug+Tr+Az+Kk Translit & Ug+Ug Translit & Ug Translit  &  89.83  &68.69&52.06&
%\hdashline
%XLM-R & selected & Ug  & Ug &  && 

\hline
% 10845293
mBERT & - &  Ug & Ug &   76.98&45.47  &24.32&

mBERT & - &  Ug+Ug-Translit & Ug &75.53   & 45.12 &28.59&
mBERT & Ug & Ug+Ug-Translit & Ug & 77.33 & 46.32& 28.84&
mBERT & Ug+Ug-Translit & Ug+Ug-Translit & Ug & 78.12 &49.32 &\bf46.01&

\hdashline
mBERT & - &  Ug Translit & Ug Translit &  87.92 & 64.98 &35.07 &
mBERT &  - & Ug+Ug Translit & Ug Translit & 88.06 &62.57& 43.60&
%mBERT &  Ug & Ug Translit &Ug Translit & 87.42 & &&
% 10879596 
mBERT &  Ug+Ug-Translit & Ug Translit &Ug Translit & \bf 89.75 & \bf 65.12 &50.57&
mBERT &  Ug+Ug-Translit & Ug +Ug Translit &Ug Translit & &64.09&\bf 55.80&

%mBERT & - & Ug-Translit & Ug-Translit &  & &to run&
\midrule
\midrule
XLM-R & - & Mt & Mt & 91.18 & 72.63 &44.32&
%XLM-R & Mt (50k) & Mt & Mt & 96.87 & 84.24 &75.45&
XLM-R & Mt (50k) & Mt & Mt & \bf 96.87 & 83.82 &75.45&
XLM-R & Mt + Ar + It & Mt & Mt & 96.57&\bf 84.31&78.53&
%XLM-R & Mt + Ar + EN & Mt & Mt & 96.81&\bf 84.22&79.22&

XLM-R & Mt + En & Mt & Mt & \underline{96.85} &\underline{84.12} &\underline{79.83}&
XLM-R & Mt + Mt translit (to Ar) & Mt & Mt & 96.45 & 82.57 &69.34&
XLM-R & Mt + Ar translit (to lat) & Mt & Mt & 96.60&80.13&71.00&






XLM-R & \textsc{select} & Mt & Mt &96.66 &83.66&\bf 81.53&
%\hdashline
%XLM-R & Mt + Ar + it & Mt+Mt shifted & Mt & &\bf  84.72&&
%XLM-R & Mt + Ar + it & Mt+Mt shifted & Mt & &\bf  84.72&&

%XLM-R & Mt + Ar + it & Mt+Mt translit(ar)  & Mt & &\bf  &&

%\hdashline
%XLM-R & Mt + Mt translit & Mt+Mt translit & Mt &&83.46&&

\midrule

\multicolumn{1}{c}{\textit{Baselines}}&&\\
\textsc{udpipe 2.0} &&Ug & Ug& 89.87 & 67.09 \\
\textsc{udify}  &&All &  Ug& 75.88 & 48.80 \\
\hline

\textsc{udpipe 2.0} &&Mt & Mt& 95.99 & 79.71\\
\textsc{udify} &&All &  Mt&  91.98 & 75.56 \\

%\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
%\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\
\bottomrule
\end{tabular}
}
%}
\caption{Performances of mBERT, XLMR and UgBERT when \textit{task-tuned} on the Uyghur (Ug) and Maltese (Mt). \hl{transliteration word mssing someswhere}
NB: Uyghur is in the pretraining corpora of XLM-R (0.4Gb) but absent from mBERT pretraining corpora\\
}
\label{tab:translit}
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}

\end{table*}


==> ug_mlm_tuning.tex <==


\begin{table}[ht!]
\footnotesize\centering
\scalebox{0.92}{ % was .7775
\begin{tabular}{lrr}
    \toprule
    %Scenario  & 
     % Source & \mbertpos  & \mbertadaptpos & $\cap$ Vocab\\
     %\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
       %Language \& Domain
      \textit{Model}&\textsc{UPOS}&\textsc{LAS} \\%& \\
     \midrule
    %\multicolumn{1}{c}{(i) \textit{zero-shot}} & \multicolumn{2}{c}{}\\
    %Zero shot Cross-lingual transfer & mBERT & fr\_gsd && 35.57  \\ 
    %Zero shot transfer &
%\midrule
%&\underline{Ref}&\underline{0-1}\\
%\multicolumn{4}{c}{\textit{\inlang}}&&&&\\

%\textsc{In} & \textsc{In} & \textsc{In} & en & 86.00 & \cellcolor{lightgreen}-0.42 \\ 
%\textit{Tasks}&\multicolumn{2}{c}{\textit{Parsing}}&\multicolumn{2}{c}{\textit{POS}}&\multicolumn{2}{c}{\textit{NER}}\\
\multicolumn{1}{c}{\textit{MLM from scratch}}\\
UgBERT (100k) & 87.39 & 57.29 \\
\midrule
\multicolumn{1}{c}{\textit{no MLM fine-tuning}}\\
\textsc{mbert } & 76.98 & 45.47\\ 
\multicolumn{1}{c}{\textit{MLM fine-tuning on 100k sentences}}\\
\textsc{mbert ug 100k} & 77.33 & 48.91 \\ 
%\textsc{mbert tr 100k} & 73.68 & 43.80 \\ 
\multicolumn{1}{c}{\textit{MLM fine-tuning on 200k sentences}}&&\\
\textsc{mbert ug 100k + tr 100k} & 76.36 & 47.19 \\ 
%\textsc{mbert az 100k} & 74.35 & 43.60 \\ 
\textsc{mbert ug 100k + tr kk az 100k} & 77.19 & 48.99 \\ 

\midrule
 \multicolumn{1}{c}{\textit{no MLM fine-tuning}}&&\\
\textsc{xlm-roberta-base} & 86.71 & 65.30 \\ 
\hdashline
\multicolumn{1}{c}{\textit{MLM fine-tuning on 100k sentences}}\\
\textsc{xlm-r ug 100k} & 88.83 & 65.49 \\ 
%\textsc{xlm-r az 100k} & 89.49 & 67.77 \\ 
\textsc{xlm-r ug 50k +en 50k} & \bf 90.27 & 68.46 \\
\textsc{xlm-r ug 50k + hu 50k} & 90.11 & 64.66 \\
\textsc{xlm-r ug 50k + tr 50} & 89.77 & 67.85 \\
\hdashline
\multicolumn{1}{c}{\textit{MLM fine-tuning on 200k sentences}}&&\\
\textsc{xlm-r ug 100k + en 100k} & 90.07 &  68.48 \\ 
\textsc{xlm-r ug 100k + tr kk az 100k} & 90.06 & 68.36 \\ 
\textsc{xlm-r ug + ug transliterated 100k} & x & \bf 69.32 \\ 
\hdashline
\multicolumn{1}{c}{\textit{MLM fine-tuning (200k) + Task-tuned on tr }}&&\\
\textsc{xlm-r ug + ug transliterated 100k} & x & \bf 70.24 \\ 
\hdashline
\multicolumn{1}{c}{\textit{Baselines}}&&\\
\textsc{udpipe 2.0} \cite{kondratyuk-straka-2019-75} &  89.87 & 67.09 \\
\textsc{udify} \cite{kondratyuk-straka-2019-75}  &  75.88 & 48.80 \\


%\textsc{\indomain} & 68.23 & \cellcolor{brightlavender}-30.59&90.89 & \cellcolor{brightlavender}-29.33& 78.57 & \cellcolor{brightlavender}-41.46\\
%\hdashline
%\multicolumn{1}{c}{ %-\textit{Out-of-Domain}}&\\
%\textsc{\outdomain} & 53.97 & \cellcolor{brightlavender}-24.31 & 90.89 & \cellcolor{brightlavender}-29.33&-&-\\

\bottomrule
\end{tabular}
}
%}
\caption{Performances of mBERT, XLMR and UgBERT when \textit{task-tuned} on the Uyghur treebank with MLM-fine-tuning on various combination of languages \\
NB: Uyghur is in the pretraining corpora of XLM-R (0.4Gb) but absent from mBERT pretraining corpora\\
\textit{Comments: (i) Broadly speaking, MLM fine-tuning, when UY sentences are included, improves downstream performances. It is more impactful on XLM-R than mBERT. \\
(ii) Combining languages does not seem to help for mBERT. For XLM-R it does help but regardless of language family (using English helps as much (or more) than using Turkish, Kazakh, Azerbaijani\\
(iii) A MLM trained from scratch is better than mBERT even with the same amount of seen Uyghur sentences. This shows the limit of unsupervised fine-tuning with such a distant language when the target is not in the pretraining corpora. 

}}
%\textbf{\textcolor{green}{$\geq$ reference} ~~ \textcolor{lightgreen}{$\leq$ reference}~~
%\textcolor{pink}{$\leq$ 2 points drop}~~
%\textcolor{red}{$\leq$ 5 points drop} ~~
%\textcolor{darkred}{$\leq$ 20 points drop}}
\label{tab:ug_mlm}
\end{table}

